Physics of stars and measurement data

Astrophysics = the star physics was beginning its development without a supporting of measurement data, which could not be obtained then. Still astrophysics exists without this support, although now astronomers collected a lot of valuable information. This is the main difference of astrophysics from all other branches of physics, for which foundations are measurement data. The creation of the theory of stars, which is based on the astronomical measurements data, is one of the main goals of modern astrophysics. Below the principal elements of star physics based on data of astronomical measurements are described. The theoretical description of a hot star interior is obtained. It explains the distribution of stars over their masses, mass-radius-temperature and mass-luminosity dependencies. The theory of the apsidal rotation of binary stars and the spectrum of solar oscillation is considered. All theoretical predictions are in a good agreement with the known measurement data, which confirms the validity of this consideration.

==> notationE.tex <==
\hspace{2cm} {\Large{The Annotation}} \vspace{1cm}



    The physics of stars requires from its models and theories to be in accordance with totality of existing astrophysical knowledge. It is basis for the star physics. This is the main difference of astrophysics from all other branches of physics, for which foundations are  measurement data.


However at an using the progress of a measuring technics, the important measurement data were obtained by astronomers for few last decades. The existence of these data gives a possibility to establish the star physics on the solid base of an agreement of the theory and data of measurements.

To reach the consent of the theory of stars with data of astronomical measurements, it is necessary to abandon to some astrophysical constructions, which are commonly accepted today. At first, necessary to take into account that the interior of the star is formed by electron-nuclear plasma - the electrically polarized medium. So the equation of the balance of plasma in gravitational field must take into account the role of the gravity-induced electric polarization. The taking into account of the gravity-induced electric polarization of plasmas allows to formulate the theory of a star, in which all main parameters - a mass of the star, its temperature, radius and luminosity - are expressed by determined combinations of the world constants, but star individuality is depended of only two parameters - mass and charge numbers of atomic nuclei from which stellar plasma is composed. This theory gives quantitative explanations with satisfactory accuracy for all dependencies, which are measured by astronomers now.


The special attention attracts the stellar mass spectrum. Theoretically the mass of the star can be calculated on a base of balance equations of the intra-stellar plasma.  It turns out that, the majority of stars, except most heavy, is composed by plasma with  neutron-excess atomic nuclei. The stability of these nuclei is attached by the specifical mechanism of neutronization acting into dense plasma.



Within the framework of this approach, the theories of the periastron rotation of close binary stars and the magnetic field of stars was considered.


It is important to note, that the taking into account of the gravity-induced electric polarization leads to the other conceptual changes. For instance, it rejects the collapse mechanism of stars at the last stage of their evolutions and hereunder puts the question about a mechanism of the "black holes" formation.


    Thereby, at taking into account the gravity-induced effects in plasma, we must refuse some models, which are commonly accepted today and seem obvious. The process of a refusing can be painful for a conservative part of astrophysical community. But this refusing is completely justified and absolutely necessary. Only herewith the quantitative explanation can be obtained for all corresponding measurement data without using of a any fitting parameter. The star physics obtains herewith the reliable foundation in the manner of result of these measurements, as a physical science must have.






